PuRe: Robust pupil detection for real-time pervasive eye tracking

Real-time, accurate, and robust pupil detection is an essential prerequisite to enable pervasive eye-tracking and its applications -- e.g., gaze-based human computer interaction, health monitoring, foveated rendering, and advanced driver assistance. However, automated pupil detection has proved to be an intricate task in real-world scenarios due to a large mixture of challenges such as quickly changing illumination and occlusions. In this paper, we introduce the Pupil Reconstructor PuRe, a method for pupil detection in pervasive scenarios based on a novel edge segment selection and conditional segment combination schemes; the method also includes a confidence measure for the detected pupil. The proposed method was evaluated on over 316,000 images acquired with four distinct head-mounted eye tracking devices. Results show a pupil detection rate improvement of over 10 percentage points w.r.t. state-of-the-art algorithms in the two most challenging data sets (6.46 for all data sets), further pushing the envelope for pupil detection. Moreover, we advance the evaluation protocol of pupil detection algorithms by also considering eye images in which pupils are not present. In this aspect, PuRe improved precision and specificity w.r.t. state-of-the-art algorithms by 25.05 and 10.94 percentage points, respectively, demonstrating the meaningfulness of PuRe's confidence measure. PuRe operates in real-time for modern eye trackers (at 120 fps).

==> Makefile <==
# USER DEFINED
RELEASE=cviu-pure
TARGET=main
READER=zathura

# DERIVED
TEX=$(TARGET).tex
OUTPUT=$(TARGET).pdf

# GIT

COMMIT=$(shell git describe --tags)

view: pdf
	$(READER) $(OUTPUT)

pdf:
	latexmk $(TARGET).tex -silent -pdf

clean:
	latexmk -C $(TARGET).tex

.PHONY: release
release:
	cp $(TARGET).pdf $(RELEASE)_$(COMMIT).pdf

.PHONY: main.detex
main.detex: main.tex
	@detex main.tex > main.detex

check: common_mistakes hyphen_check article_check

common_mistakes:
	./scripts/common_mistakes.sh

hyphen_check:
	./scripts/hyphen_check.sh

article_check: main.detex
	detex main.tex | ./scripts/article_check.py

cviu-release:
	rm -rf release
	mkdir release
	cp main.tex release/
	sed -i 's/\\input{src\//\\input{/g' release/main.tex
	cp macros.tex release/
	cp refs.bib release/
	cp Makefile release/
	cp elsarticle.cls release/
	cp ycviu.sty release/
	cp model2-names.bst release/
	cp src/* release/
	grep includegraph release/* | ./copy-graphics.py

split:
	pdftk main.pdf cat 1 output authorship-confirmation.pdf
	pdftk main.pdf cat 2 output graphical-abstract.pdf
	pdftk main.pdf cat 3 output highlights.pdf
	pdftk main.pdf cat 4-end output manuscript.pdf


==> graphical-abstract.tex <==
\begin{table*}[!th]
\ifpreprint\else\vspace*{-5pc}\fi

\section*{Graphical Abstract (Optional)} To create your abstract, please type over the instructions in the
template box below.  Fonts or abstract dimensions should not be changed
or altered.

\vskip1pc
\fbox{
\begin{tabular}{p{.4\textwidth}p{.5\textwidth}}
\bf PuRe: Robust pupil detection for real-time pervasive eye tracking  \\
Thiago Santini, Wolfgang Fuhl, Enkelejda Kasneci\\[1pc]
\includegraphics[width=0.9\textwidth]{imgs-graphical-abstract-test.pdf}%%.pdf
&
%}\\
\end{tabular}
}

\end{table*}
\clearpage


==> highlights.tex <==
\begin{table*}[!t]
\ifpreprint\else\vspace*{-15pc}\fi

\section*{Research Highlights (Required)}

To create your highlights, please type the highlights against each
\verb+\item+ command.

\vskip1pc

\fboxsep=6pt
\fbox{
\begin{minipage}{.95\textwidth}
It should be short collection of bullet points that convey the core
findings of the article. It should  include 3 to 5 bullet points
(maximum 85 characters, including spaces, per bullet point.)
\vskip1pc
\begin{itemize}

 \item A novel computer-vision based algorithm for robust pupil detection is introduced

 \item The algorithm increases detection rate up to ten percentage points in challenging data

 \item Additional evaluation metrics for pupil detection algorithms are introduced

 \item Specificity, precision, and sensitivity improved by 5.96\%, 25.05\%, and 10.94\%

 \item The algorithm runs in real time for modern eye trackers (at 120 fps)

\end{itemize}
\vskip1pc
\end{minipage}
}

\end{table*}

\clearpage

